The Role of Variability in Human-Machine Interaction Experience

Human-machine interaction (HMI) requires control strategies that account for the nature of human motor behavior. Conventional shared-control and haptic-assistance methods typically ignore the stochastic nature of human behavior, potentially limiting both performance and human interaction experience. In this study, we designed an experimental setting and evaluated a novel human-variability-aware optimal controller. Participants performed a physically coupled haptic interaction task in three conditions: a controller mode that aims at conventionally reducing overall variability, a variability-aware controller mode designed to maintain human natural variability patterns, and a human-only control condition serving as a baseline. We analyzed behavioral variability, task performance, and human interaction experience. The results show that considering natural movement variability significantly increased perceived interaction quality in terms of usability while maintaining task performance. These findings highlight the importance of incorporating stochastic human movement characteristics into shared-control designs and demonstrate the feasibility and benefits of the proposed control strategy for human-centered control design of HMI.

==> 1_tex/00_myConfig.tex <==
% The following packages can be found on http:\\www.ctan.org
\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{epsfig} % for postscript graphics files
%\usepackage{mathptmx} % assumes new font selection scheme installed
%\usepackage{times} % assumes new font selection scheme installed
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{xcolor}
\usepackage{nicefrac}
\usepackage{siunitx}


%packages sean
%\usepackage[shortlabels]{enumitem}
\usepackage{tabularray}
\UseTblrLibrary{amsmath} %for colsep=-2
\usepackage{caption}
\usepackage{subcaption}
\usepackage{xspace}
\usepackage{placeins}

%Packages Jan
\usepackage{tikz}
\usetikzlibrary{arrows.meta}
\sisetup{
    locale=UK,
    output-decimal-marker={.},
  separate-uncertainty = true
}

%Theorems:
\usepackage[noconfig,amsmath,thmmarks]{ntheorem}
\theoremnumbering{arabic}
\theoremstyle{plain}
\RequirePackage{latexsym}
\theorembodyfont{\itshape}
\theoremheaderfont{\normalfont\bfseries}
\theoremseparator{}
\newtheorem{assumption}{Assumption}
\newtheorem{remark}{Remark}
\newtheorem{problem}{Problem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
%\newtheorem{proof}{Proof}

\usepackage{tikz}
\usepackage{pgfplots}
%\usepackage{cite}
\usepackage{makecell}
\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}
\newcommand{\notiz}[1]{\textcolor{gray}{note: #1}}
\newcommand{\plotTodo}[1]{\textcolor{blue}{PLOT: #1}}


%math commands
\newcommand{\bm}[1] {\boldsymbol{#1} }
\newcommand{\cov}[2]{\mathrm{cov}\left( #1, #2\right)}
\newcommand{\covs}[1]{\mathrm{cov}\left( #1 \right)}
\newcommand{\E}[1]{\mathrm{E}\left\{#1\right\}}
\newcommand{\mat}[1]{\left[\begin{matrix} #1 \end{matrix}\right]}
\newcommand{\Var}[1]{\mathrm{Var}\left(#1\right)}
\newcommand{\mean}[1]{\mathrm{mean}\left(#1\right)}
%\newcommand{\comment}[1]{\textcolor{gray}{#1}}
\newcommand{\Comment}[1]{\textcolor{red}{#1}}
\newcommand{\commentBalint}[1]{\textcolor{blue}{#1}}



%VARS SEAN
\newcommand{\nosup}{\textit{noSup}\xspace}
\newcommand{\highvar}{\textit{highVar}\xspace}
\newcommand{\lowvar}{\textit{lowVar}\xspace}


\newcommand{\posvar}{V_y}
\newcommand{\posvarmax}{V_y^{\mathrm{max}}}
\newcommand{\posvarend}{V_y^{\mathrm{end}}}

%alt
%\newcommand{\posvar}{\overline{\Var{\bm{p}_y}}}
%\newcommand{\posvarmax}{\overline{\Var{\bm{p}_y}}_{\mathrm{max}}}
%\newcommand{\posvarend}{\overline{\Var{\bm{p}_y}}_{\mathrm{end}}}
\newcommand{\poserrend}{\overline{e}_{\mathrm{end}}}
